Towards a Scalable Reference-Free Evaluation of Generative Models

While standard evaluation scores for generative models are mostly reference-based, a reference-dependent assessment of generative models could be generally difficult due to the unavailability of applicable reference datasets. Recently, the reference-free entropy scores, VENDI and RKE, have been proposed to evaluate the diversity of generated data. However, estimating these scores from data leads to significant computational costs for large-scale generative models. In this work, we leverage the random Fourier features framework to reduce the computational price and propose the Fourier-based Kernel Entropy Approximation (FKEA) method. We utilize FKEA's approximated eigenspectrum of the kernel matrix to efficiently estimate the mentioned entropy scores. Furthermore, we show the application of FKEA's proxy eigenvectors to reveal the method's identified modes in evaluating the diversity of produced samples. We provide a stochastic implementation of the FKEA assessment algorithm with a complexity $O(n)$ linearly growing with sample size $n$. We extensively evaluate FKEA's numerical performance in application to standard image, text, and video datasets. Our empirical results indicate the method's scalability and interpretability applied to large-scale generative models. The codebase is available at https://github.com/aziksh-ospanov/FKEA.

==> Paper-text/0-abstract.tex <==
%Standard evaluation scores for generative models are mostly reference-based and quantify the generative models' properties compared to a reference distribution. However, a reference-dependent assessment of prompt-based generative models could be difficult due to the lack of applicable reference datasets.
While standard evaluation scores for generative models are mostly reference-based, a reference-dependent assessment of generative models could be generally difficult due to the lack of applicable reference datasets. 
%To address the need for reference-free evaluation metrics
Recently, the reference-free entropy scores, VENDI \cite{friedman_vendi_2023} and RKE \cite{jalali_information-theoretic_2023}, have been proposed to evaluate the diversity of generated data. Nevertheless, estimating these scores from data leads to significant computational costs for large-scale generative models. In this work, we leverage the Random Fourier Features framework to reduce the metrics' complexity and propose the \emph{Fourier-based Kernel Entropy Approximation (FKEA)} method. We utilize FKEA's approximated eigenspectrum of the kernel matrix to efficiently estimate the mentioned entropy scores. Furthermore, we show the application of FKEA's proxy eigenvectors to reveal the method's identified modes in evaluating the diversity of produced samples. %We theoretically support the FKEA framework by proving that the required Fourier feature size grows only logarithmically with the sample size $n$,  while computing the original entropy scores would demand at least $O(n^2)$ computations. 
%the \emph{truncated kernel entropy scores} using only the top-$t$ principal eigenvalues for the entropy calculation. We subsequently propose the application of Random Fourier Features (RFFs) to perform an efficient estimation of the kernel-based entropy scores, resulting in a scalable reference-free evaluation method which we call \emph{Fourier-based Kernel Entropy Approximation (FKEA)}. 
%We prove that the number of Fourier features required for a proper approximation of entropy scores grows only logarithmically with the sample size $n$, showing the accuracy of FKEA under a limited Fourier feature size. 
We provide a stochastic implementation of the FKEA assessment algorithm with a complexity $O(n)$ linearly growing with sample size $n$. We extensively evaluate FKEA's numerical performance in application to standard image, text, and video datasets. Our empirical results indicate the method's scalability and interpretability applied to large-scale generative models.     

==> Paper-text/1-introduction.tex <==
A principled comparison of generative models requires evaluation metrics to quantify the quality and diversity of the models' produced data. Since the introduction of variational autoencoders (VAEs) \cite{kingma_auto-encoding_2013} and generative adversarial networks (GANs) \cite{goodfellow_generative_2014} that led to impressive empirical results in application to image data, most of the standard assessment scores were originally developed for image-based generative models. As the application of generative model frameworks expanded to other domains such as text and video data, the machine learning community has attempted to adapt the established image-based scores to the non-image target domains. While such extensions of the image-based evaluation criteria have been successful and widely adopted in several cases, recent studies \cite{gao2024llm,shaib2024standardizing} have reported challenging instances of applying standard evaluation scores to assess large-scale text and video-based generative models.     
%the extension of the image-based evaluation criteria to state-of-the-art text and video generative models has been the focus of several recent studies.

An important challenge in extending the image-based evaluation scores to a general case is their reference-based definition, i.e., they quantify the properties of a generative model in comparison to a reference distribution of data. Therefore, the reference distribution, which is often chosen to be the distribution of samples in the test dataset, plays a central role in the assessment. Specifically, the distance-based metrics, Fréchet Inception Distance (FID) \cite{heusel_gans_2018} and Kernel Inception Distance (KID) \cite{binkowski2018demystifying}, are explicitly reference-based, measuring the distance between the generative and reference distributions. Similarly, the standard quality/diversity score pairs, precision/recall \cite{sajjadi_assessing_2018,kynkaanniemi_improved_2019} and density/coverage \cite{naeem_reliable_2020}, perform the evaluation in comparison to a reference dataset. Even the seemingly reference-free Inception Score \cite{salimans_improved_2016} can be viewed as implicitly reference-based, since it quantifies the variety and fidelity of data based on the labels and confidence scores assigned by an ImageNet \cite{deng2009imagenet} pre-trained model, where ImageNet implicitly plays the role of the reference distribution. Note that the reference-based nature of these evaluation metrics is desired in evaluating standard image-based generative models, where either a sufficiently large test sample set or a comprehensive reference dataset such as ImageNet is available for the reference-based evaluation.    

On the other hand, a reference-dependent assessment of generative models may not always be feasible, because the selection of a reference distribution could be difficult in a general learning scenario. Especially, in prompt-based generative models where the data are created in response to a user's input text prompts, the generated data would follow an a priori unknown distribution depending on the specific distribution of the user's input prompts. Consequently, a proper reference-based evaluation for every user's generated data would require a distinct reference dataset, which may not be available to the user in the assessment time. Moreover, finding a comprehensive text or video dataset to play the role of the reference distribution would be more challenging compared to the case of image data, because the higher length of the text and video samples could significantly contribute to their variety, requiring an inefficiently large reference set to cover all sample types.

The discussed challenges of a reference-based evaluation of generative models highlight the need for reference-free assessment methods that remain functional in the absence of a reference dataset. Recently, two entropy-based diversity evaluation scores, the VENDI \cite{friedman_vendi_2023} and RKE \cite{jalali_information-theoretic_2023} metrics, have been proposed in the literature to address the need for reference-free assessment metrics. Based on the theoretical results in \cite{jalali_information-theoretic_2023}, the evaluation process for these scores can be viewed as an unsupervised identification of the generative model's produced sample clusters, followed by the entropy calculation for the frequencies of the detected clusters. Assuming that the identified clusters are semantically meaningful, the VENDI and RKE scores provide an information-theoretic quantification of the cluster-based diversity.

While the VENDI and RKE entropy scores offer reference-free assessments of generative models, estimating these scores from finite generated data
could demand significant computational and statistical costs. In this work,  
 we prove that computing the precise RKE and Vendi scores would demand respectively $\Omega (n^2)$ and $\Omega (n^{2.376})$ computations for a sample size $n$. %In practice, interpreting the methods via the eigenvectors of the kernel matrix requires applying eigendecomposition algorithms to the $n\times n$ kernel matrix leading to $O(n^3)$ computations. 
Therefore, the method's application to large-scale generative models and datasets with hundreds of sample types would remain largely infeasible. Furthermore, we show that estimating the VENDI score from empirical data requires $\Omega(d)$ samples for a kernel feature map size $d$, which could be significantly large for the standard Gaussian kernel with a potentially infinite feature map size.

To overcome the challenges of estimating the entropy scores, we leverage the framework of random Fourier features (RFFs) \cite{rahimi_random_2007} and develop a scalable entropy-based evaluation method that can be efficiently applied to large sample sizes. Our proposed method, \emph{Fourier-based Kernel Entropy Approximation (FKEA)}, is designed to approximate the kernel covariance matrix using the RFFs drawn from the Fourier transform-inverse of a target shift-invariant kernel. We prove that using a Fourier feature size $r=\mathcal{O}\bigl(\frac{\log n}{\epsilon^2}\bigr)$, FKEA computes the eigenspace of the kernel matrix within an $\epsilon$-bounded approximation error. We show this guarantee translates into an $\mathcal{O}\bigl(\sqrt{\frac{\log n}{r}}\bigr)$-accurate approximation of the RKE score. Also, we demonstrate that the FKEA approximation guarantee can be extended to a truncated version of VENDI score, measuring the entropy of the top $t$ eigenvalues, resulting in an $\mathcal{O}\bigl(\sqrt{\frac{t\log n}{r}}\bigr)$-accurate approximation of the $t$-truncated VENDI score. %Furthermore, we prove that our defined $t$-truncated VENDI score can effectively reduce the sample complexity of VENDI score, as we numerically show the significant VENDI score's sample complexity under the high-dimensional Gaussian kernel, while the sample complexity of $t$-truncated VENDI seems smaller in the experiments.  

Furthermore, we utilize the eigenvectors of the FKEA's proxy kernel covariance matrix for interpreting the reference-free evaluation process. Our theoretical analysis suggests the correspondence between the FKEA's found eigenvectors and the mean of the distribution modes identified by the kernel-based assessment method. We prove that the Gaussian kernel-based FKEA will possess an exclusive eigendirection for every distribution mode, if the mode has a higher self-variance than its covariance with the remaining component of the generative model. Therefore, the evaluator can interpret the reference-free diversity quantification by investigating the sample clusters corresponding to the FKEA's proxy eigenvectors. 

Finally, we numerically analyze the reference-free entropy-based evaluation of generative models using the baseline eigendecomposition-based and our proposed FKEA methods. We empirically show that whereas the baseline method cannot efficiently scale to sample sizes beyond a few ten thousands, the FKEA method could scalably apply to large-scale sample sets, following our proposed fully stochastic implementation of the FKEA method. Utilizing the recent embeddings of image, text, and video data, we test the FKEA assessment and compute the sample clusters and their frequencies in application to large-scale computer vision and natural language processing datasets and generative models. Given the powerful deep neural net-based embeddings of the input image and text data, we observe that the reference-free FKEA method can detect semantically meaningful sample clusters at a relatively low computational cost, offering a scalable reference-free assessment of the models. In summary, the following are our work's main contributions:

\begin{itemize}[leftmargin=*]
    \item Characterizing computational complexity bounds for the kernel entropy-based evaluation scores of generative models
    \item Developing the stochastic Fourier-based FKEA method to approximate the kernel covariance eigenspace and entropy of the generated data
    \item Proving guarantees on FKEA's required size of random Fourier features indicating a complexity logarithmically growing with the dataset size
    \item Providing numerical results on FKEA's reference-free assessment of large-scale image,text, video-based datasets and generative models.
\end{itemize}



==> Paper-text/9-Checklist.tex <==
\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper discusses and further expands the ideas of generative model entropic diversity evaluation presented in the abstract and introduction.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In the paper we discuss the limitations of the reference-free metrics (RKE, VENDI) approximation via the Random Fourier Features within Fourier-based Kernel Entropy Approximation (FKEA) method.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper provides preliminary information, assumptions and definitions of the theoretical results along with relevant proofs. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper outlines all necessary parameters in experimental settings for reproducibility purposes.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The submission comes along with demo code to generate clusters and compute the scores.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Each experimental result is accompanied by relevant parameters that aid in understanding of presented results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Error bars are not reported due to limited amount of ground truth samples in the datasets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper states the computational resources used in the experimental setups.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper closely follows the code of ethics and all generated/downloaded data has through sanity checks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper discuss computational complexity and diversity evaluation of existing metrics (RKE, VENDI) and does not directly impact training of models.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In this paper we discuss the evaluation of existing datasets and generative models. We do not release any custom datasets to the public.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All relevant datasets and models are referenced in the paper and supplemental materials.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not release new assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve human evaluation and crowdsourcing.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve human evaluation and crowdsourcing.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}
